Bifrost: Secure, Scalable and Efficient File Sharing System Using Dual Deduplication

We consider the problem of sharing sensitive or valuable files across users while partially relying on a common, untrusted third-party, e.g., a Cloud Storage Provider (CSP). Although users can rely on a secure peer-to-peer (P2P) channel for file sharing, this introduces potential delay on the data transfer and requires the sender to remain active and connected while the transfer process occurs. Instead of using the P2P channel for the entire file, users can upload information about the file on a common CSP and share only the essential information that enables the receiver to download and recover the original file. This paper introduces Bifrost, an innovative file sharing system inspired by recent results on dual deduplication. Bifrost achieves the desired functionality and simultaneously guarantees that (1) the CSP can efficiently compress outsourced data; (2) the secure P2P channel is used only to transmit short, but crucial information; (3) users can check for data integrity, i.e., detect if the CSP alters the outsourced data; and (4) only the sender (data owner) and the intended receiver can access the file after sharing, i.e., the cloud or no malicious adversary can infer useful information about the shared file. We analyze compression and bandwidth performance using a proof-of-concept implementation. Our experiments show that secure file sharing can be achieved by sending only 650 bits on the P2P channel, irrespective of file size, while the CSP that aids the sharing can enjoy a compression rate of 86.9 %.

==> sections/rel_work.tex <==
% To allow compilation of the file
% !TeX root = ./../Yggdr.tex

\section{Related Work}
\label{sec:relwork}


==> sections/transformations.tex <==
% To allow compilation of the file
% !TeX root = ./../Yggdr.tex
\subsection{Allowed Transformations in \name}\label{sec:transformations}
From information theory, we know four functions to transform a string.
Namely, \begin{enumerate*}[label=(\roman*)]
\item \label{lins} insert an element to a position,
 \item \label{ldel} delete an element from a position, 
 \item \label{lswap}
  swap two elements, and 
 \item \label{lchange}
 change the value of a given position.
\end{enumerate*}
%functions to apply on the data to generate a number of possible transformations for our generalized deduplication approach.
%In order to have efficient deduplication, we also define some policies. In this section we take a look at the funtions and policies we use in our setup. 
%Throughout this work, we consider our data to be strings of a fixed length.
%we can use 4 functions to transform a string. These functions are as follows:
% \begin{enumerate}
% 	\item Insert an element to a position.
% 	\item Delete an element from a position.
% 	\item Swap two consecutive elements.
% 	\item Change the value of a position.
% \end{enumerate}
%The difference between these functions is 
%Note that swap and change value do not change the length of the string, while insert and delete do. %operations change the length of the string.

\name allows \user and \cloud to determine policies on how to transform the data to obtain deduplication friendly strings. 
The aim is to minimize the number of functions to perform while achieving efficient deduplication rate on the Cloud and some level of privacy at the Clients. 
%Minimizing the number of operations increases the compression potential as the generated deviation needs to be stored to recover the original data.
%We provide policies on how to combine the aforementioned transformations %(denoted by $\mathcal{T}$) 
These policies typically require a metric to determine similarity among strings. 
%A natural metric is 
%As mentioned in section~\ref{intro}, the deduplication procedure can be performed on string that are nearly identical. The similarity between the strings is measured by one of the following metrics.
The \textbf{Hamming distance} indicates the number of positions with different values in two strings of the same length. 
%This essentially tells us how many 
which is equal to the number of \emph{change value} operations needed to transform a string into another. \textbf{Swap Distance} indicates the number of operations to change a string into another using only the \emph{swap} and \emph{change value}.
\textbf{Damerau–Levenshtein Distance} is the most complete metric, indicating the number of operations to transform one string into another if we use all 4 transformations \ref{lins}-\ref{lchange}~\cite{brill2000improved}.
% \begin{enumerate}
% 	\item \textbf{Hamming Distance}: The number of positions at which the corresponding symbols are different. This distance is only applicable for two strings of the same length. Hamming distance shows the number of operations we need to do to transform one string into another string if we only use the change value function.
% 	\item \textbf{Swap Distance}: The number of operations to transform one string to another one if we only use change value and swap functions.
% 	\item 
% 	\textbf{Damerau–Levenshtein distance}: The number of operations to transform one string into another if we use all 4 functions.
% \end{enumerate}

Previous work on GD focused primarily on change value operations using Hamming or Reed-Solomon Codes~\cite{rasmus,Vestergaard2019b}. 
%In these works, the notion of closeness is the Hamming Distance.
%In this work, 
Here we instead consider the three operations \ref{ldel}-\ref{lswap}-\ref{lchange}: delete (\deletions), swap (\swap) and change value (\changev). 
We discard the \emph{insert} function as it increases the size of a string, which is counterproductive for compressing the data.
%In previous works of the generalized deduplication, the hamming codes was used to ensure deduplication. In this sense, the original string is transformed to the basis with the lowest hamming distance. In this case, the bases were pre-defined~\cite{rasmus}. However, in this work, we use the swap distance in order to transform the generated bases into bases that can be deduplicated. The swap distance is more general and allows defining the bases with respect to data instead of using pre-defined bases.

In \name, 
%we use one transformation policy for \user and one for \cloud. The 
\user applies \deletions transformations on \file prior to upload to achieve the desired level of privacy.
This transformation acts as a deletion channel~\cite{mitzenmacher2009} for the \cloud.
% (who gets the punctured string $\file'$). 
% Determining the original data chunk is a hard problem.
%, even if it could control the encoding of the original data before introducing it to the channel (which is not the case in our application).
%The hardness of the reconstruction of the original data reflects into the \user's privacy level.
\cloud applies \swap and \changev to reduce the distance between the strings uploaded by \user, generating strings that are suitable for deduplication. 
%In this work, we use some policies in order to ensure efficient deduplication on the cloud, i.e., to ensure that the bases can be transformed using the minimum number of operations. To achieve this goal, we need to generate strings with the swap distance of less than a certain threshold. As the bases are generated by deletion operation, we need to define some policies to ensure lower swap distance. 

%In order to define the policies, we need to identify the characteristics which reduce the expected swap distance between a set of strings. In general, we are interested to generate strings that can be transformed into other strings by swaps, because each swap changes the value of two elements, while change value only changes the value of one element. One of the possible ways to reduce the expected swap distance is to generate strings with a fixed probability distribution on the values. In this case, the probability of having the same amount of a value in different strings is close, hence, intuitively, less number of operations is needed to perform deduplication on the strings.

%Using these operations and policies, we can now define our system model and the proposed algorithm for generalized deduplication.

% Figure~\ref{dataFig} provides an example of a $1$-deletion transformation, where the system takes the element in the sixth position (with value $1$) and deletes it from the string.
% The resulting string will be the basis of the transformation.
% A short description of the change (a pair indicating the element deleted and position: $(1,6)$) constitutes the deviation.
% Note that multiple $1$-deletion operations can be carried out.
% As long as the deviation is applied in the correct order, the original data can be recovered.

%\begin{itemize}
%	\item Deletion of 1 element.
	%	\item Deletion of $y > 1$ elements, i.e., $y$-deletion.
%	\item Swapping two elements.%
%	\item Changing a value of an element.
%\end{itemize}

% \begin{figure*}[t]
% 	\centering
% 	\begin{tikzpicture}[
% 	node distance=0pt,
% 	start chain = A, %going right,
% 	X/.style = {rectangle, draw,% styles of nodes in string (chain)
% 		minimum width=2ex, minimum height=3ex,
% 		outer sep=0pt, on chain},

%               B/.style = {decorate,
% 		decoration={brace, amplitude=5pt,
% 			pre=moveto,pre length=1pt,post=moveto,post length=1pt,
% 			raise=1mm,
% 			#1}, % for mirroring of brace, if necessary
% 		thick},
% 	B/.default=mirror, % by default braces are mirrored
% 	]
% 	\foreach \i in {4,6,1,3,0,7,1,2,2,
% 		5,4}
% 	\node[X,right] {\i};
	
% 	\node (end)[X, right] {5};
% 	\node (begin)[X, right = 1cm] {4};
	
% 	\foreach \i in {6,1,3,0,7,2,2,
% 		5,4,5}
% 	\node[X, right] {\i};
	
% 	\node[X,right = 0.3 cm]{1};
	
% 	\node[X, right] {6};
	
% 	\draw [arrow] (end)  -- (begin);
% 	\node (B1) [inner sep=1pt,above=of A-6.north west] {Original Data};
% 	\node (B2) [inner sep=1pt,above=of A-19.north west] {Data to Outsource};
% 	\node (B3) [inner sep=1pt,above=of A-25.north west] {Deviation};
% 	\end{tikzpicture}
% 	\caption{A simple example of a 1-deletion Transformation}
% 	\label{dataFig}
% \end{figure*}

%After the transformation is carried out, the user saves the deviation in its local memory and sends the basis to the cloud. Each of this transformations add a block to the deviation but reduces the size of the basis. Hence, increasing the number of transformations increases the storage required in the user, but reduces the storage on the cloud as the cloud is able to perform deduplication more efficiently. 

%In this paper, we are going to cover the compression ratio and some other metrics of this system. Before we define these terms, we need to set the notations used in this paper. The notation used can be seen in table~\ref{NotationTable}. 

% The strings that make the original data are consisted of a fixed length of $n_{o}$ symbols, where each symbol in the string is $k$ bits. After the trasnformations are carried out, the generated bases all have a fixed length of $n_{b}$, where $n_{b} \leq n_{o}$. This assumptions measn that the number of deletion operation that is executed on each original string is a fixed value and is equal to $n_{o} - n_{b}$.

% Using this notation, the size of each original string and basis is equal to $s_{o} = k\cdot n_{o}$ and $s_{b} = n_{b}\cdot k$ respectively. Also note that always $r \leq 1$. Number of possible values for each element is equal to $N = 2^{k}$. 

%We assume that the transformation of the data to bases and deviations are done in a way that size of the deviations are the same for each original data. Which means the operations on each original string are exactly the same. For example, we delete one element from each string three times, i.e., three 1-deletions. This assumption ensures that all bases and deviations are of the same size.



% \begin{table*}[!h]
% 	\centering
% 	\caption{Notation. Definition of the symbols used through the paper.}
% 	\label{NotationTable}\label{tab:notation}
% 	\begin{tabular}{|c|c|c|}
% 		\hline
% 		Symbol & Unit & Definition \\ 
% 		\hline
% 		$k$ & bit & Size of each element in the original strings and the bases. \\
% 		$\mathcal{N}_{o}$ & - &Number of original strings.		 \\
% 		$\mathcal{N}_{b}$ & - & Number of the bases. \\
% 		%$s_{o}$ & bit &size of original strings. \\
% 		%$s_{b}$ & bit & size of the bases. \\
% 		$n_{o}$ & - & Number of elements in the string. \\
% 		$n_{b}$ & - & Number of elements in the basis. \\
% 		$s_{d}$ & bit & size of each deviation. \\
% 		%$N = 2^k$ & - & Number of possible values for each element. \\
% 		$ r = \frac{\mathcal{N}_{b}}{\mathcal{N}_{o}}$ & - & Fraction of number of bases with respect to number of original strings. \\
% 		\hline
% 	\end{tabular}
% \end{table*}

